Stream-DiffVSR: Low-Latency Streamable Video Super-Resolution via Auto-Regressive Diffusion

Diffusion-based video super-resolution (VSR) methods deliver strong perceptual quality but are often unsuitable for latency-sensitive scenarios due to reliance on future frames and expensive multi-step denoising. We propose Stream-DiffVSR, a causally conditioned diffusion framework for efficient online VSR. Operating strictly on past frames, Stream-DiffVSR integrates a four-step distilled denoiser for fast inference, an Auto-regressive Temporal Guidance (ARTG) module that injects motion-aligned cues during latent denoising, and a lightweight temporal-aware decoder with a Temporal Processor Module (TPM) to enhance detail and temporal coherence. Unlike chunk-wise streaming inference, our strictly frame-by-frame causal design avoids sequence-level waiting, substantially reducing time-to-first-frame and end-to-end latency. Stream-DiffVSR processes 720p frames in 0.328 seconds on an RTX 4090 and consistently outperforms prior diffusion-based baselines. Compared with the online state-of-the-art TMP, it improves perceptual quality (LPIPS +0.095). Compared with prior diffusion-based VSR methods such as MGLD-VSR, it reduces per-frame runtime by over 130x. Moreover, Stream-DiffVSR substantially lowers time-to-first-frame for diffusion-based VSR, reducing initial delay from over 4600 seconds to 0.328 seconds, making diffusion-based VSR markedly more practical for low-latency online and streaming deployment. Project page: https://jamichss.github.io/stream-diffvsr-project-page/

==> algo/unet_random_timestep_distillation.tex <==
% \begin{algorithm}[t]
% \caption{Training procedure for Unet}
% \label{alg:vsr_training}
% \footnotesize
% \KwIn{Dataset $\mathcal{D}$ with (LQ, HQ) pairs, pre-trained VAE, U-Net, noise scheduler, and optional discriminator.}
% \tcp{Initialization: Set hyperparameters, load data, and initialize models.}

% \For{$epoch = 1$ \KwTo $N_{\text{epochs}}$}{
%     \For{each batch $(\text{LQ}, \text{GT})$ in dataloader}{
%         \tcp{Normalize images and upscale LQ}
%         $\text{GT} \gets 2 \times \text{GT} - 1$, \quad $\text{LQ} \gets 2 \times \text{LQ} - 1$ \;
%         $\text{upscaled\_LQ} \gets \text{BicubicUpsample}(\text{LQ}, \times 4)$ \;

%         \tcp{Select center frame}
%         $\text{GT}_0 = \text{GT}[:, T/2, ...]$, \quad $\text{LQ}_0 = \text{LQ}[:, T/2, ...]$ \;

%         \tcp{Encode ground truth into latent space}
%         $\mathbf{z}_0 = \text{VAE.encode}(\text{GT}_0)$ \;

%         \tcp{Sample noise and timesteps}
%         $\mathbf{\epsilon} \sim \mathcal{N}(0, I)$, \quad $t \sim \{249, 499, 749, 999\}$ \;

%         \tcp{Apply forward diffusion}
%         $\mathbf{z}_t = \alpha_t \mathbf{z}_0 + \sqrt{1 - \alpha_t} \mathbf{\epsilon}$ \;

%         \tcp{Concatenate noisy latent with LQ}
%         $\mathbf{\hat{z}}_t = [\mathbf{z}_t, \text{LQ}_0]$ \;

%         \tcp{Predict noise}
%         $\mathbf{\hat{\epsilon}} = \text{U-Net}(\mathbf{\hat{z}}_t, t)$ \;

%         \tcp{Compute latent-space loss}
%         $\mathcal{L}_{\text{latent}} = \|\mathbf{\epsilon} - \mathbf{\hat{\epsilon}}\|^2$ \;

%         \tcp{Decode predicted latent}
%         $\hat{\text{GT}}_0 = \text{VAE.decode}(\mathbf{\hat{z}}_0)$ \;

%         \tcp{Compute reconstruction losses}
%         $\mathcal{L}_{\text{pixel}} = \text{Charbonnier}(\hat{\text{GT}}_0, \text{GT}_0)$ \;
%         $\mathcal{L}_{\text{LPIPS}} = \text{LPIPS}(\hat{\text{GT}}_0, \text{GT}_0)$ \;

%         \tcp{Total reconstruction loss}
%         $\mathcal{L}_{\text{rec}} = \mathcal{L}_{\text{latent}} + \lambda_{\text{pixel}} \mathcal{L}_{\text{pixel}} + \lambda_{\text{LPIPS}} \mathcal{L}_{\text{LPIPS}}$ \;

%         \If{GAN loss is enabled and step $\%$ 5 == 0}{
%             \tcp{Train discriminator}
%             Compute $\mathcal{L}_{\text{D}}$ using real and fake logits \;
%             Compute adversarial loss for U-Net: $\mathcal{L}_{\text{GAN}} = \text{softplus}(-\text{D}(\hat{\text{GT}}_0))$ \;
%             Compute weight $\lambda_{\text{GAN}}$ \;
%             \tcp{Compute total loss}
%             $\mathcal{L} = \mathcal{L}_{\text{rec}} + \lambda_{\text{GAN}} \mathcal{L}_{\text{GAN}}$ \;
%         }
%         \Else{
%             $\mathcal{L} = \mathcal{L}_{\text{rec}}$ \;
%         }

%         \tcp{Update U-Net parameters using gradient descent}
%     }
% }
% \end{algorithm}

\begin{algorithm}[h]
\caption{Training procedure for U-Net distillation with random timestep selection}
\label{alg:unet_random_timestep_distillation}
\footnotesize
\KwIn{Dataset \(\mathcal{D}=\{(\tilde{I}, I)\}\); pre-trained VAE; noise scheduler; student U-Net with parameters \(\theta\); discriminator \(D(\cdot)\).}
\For{epoch \(=1\) to \(N\)}{
  \For{each batch \((\tilde{I}, I) \in \mathcal{D}\)}{
    \(\mathbf{z}_0 \gets \mathrm{VAE.encode}(I)\)\;
    Sample noise \(\epsilon \sim \mathcal{N}(0,I)\)\;
    Select a timestep \(t \sim \mathcal{U}\{999,\,749,\,499,\,249\}\)\;
    \(\mathbf{z}_t \gets \alpha_t\,\mathbf{z}_0 + \sqrt{1-\alpha_t}\,\epsilon\)\;
    
    \tcp{--- Predict noise at random timestep ---}
    \(\hat{\mathbf{z}}_t \gets [\,\mathbf{z}_t,\,\tilde{I}]\)\;
    \(\hat{\epsilon} \gets \mathrm{U\!-\!Net}(\hat{\mathbf{z}}_t, t)\)\;
    \(\mathcal{L}_{\mathrm{latent}} \gets \|\epsilon - \hat{\epsilon}\|_2^2\)\;
    
    \tcp{--- Approximate reconstruction from predicted noise ---}
    \(\hat{\mathbf{z}}_0 \gets \mathrm{Scheduler.get\_approx}(\hat{\epsilon}, t, \mathbf{z}_t)\)\;
    \(\hat{I} \gets \mathrm{VAE.decode}(\hat{\mathbf{z}}_0)\)\;
    
    \tcp{--- Loss terms ---}
    \(\mathcal{L}_{\mathrm{L2}} \gets \|\hat{I} - I\|_2^2\)\;
    \(\mathcal{L}_{\mathrm{LPIPS}} \gets \mathrm{LPIPS}(\hat{I}, I)\)\;
    \(\mathcal{L}_{\mathrm{rec}} \gets \mathcal{L}_{\mathrm{latent}} + \lambda_{L2}\,\mathcal{L}_{\mathrm{L2}} + \lambda_{\mathrm{LPIPS}}\,\mathcal{L}_{\mathrm{LPIPS}}\)\;
    \(\mathcal{L}_{\mathrm{GAN}} \gets \mathrm{softplus}\bigl(-D(\hat{I})\bigr)\)\;
    \(\mathcal{L} \gets \mathcal{L}_{\mathrm{rec}} + \lambda_{\mathrm{GAN}}\,\mathcal{L}_{\mathrm{GAN}}\)\;

    Update parameters: \(\theta \gets \theta - \eta \nabla_{\theta} \mathcal{L}\)\;
  }
}
\end{algorithm}


==> figs/rebuttal_videolq_visual.tex <==
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\columnwidth]{figs/figures/rebuttal/VideoLQ-visual.pdf}
%     \vspace{-6mm}
%     \caption{
%     \textbf{Qualitative comparison on REDS4 and Vimeo-90K-T datasets.}}
%     \label{fig:rebuttal_videolq_visual}
% \end{figure}

==> rebuttal/figs/flashvsr_ours_comparison.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth,height=0.7\columnwidth,keepaspectratio]{rebuttal/figs/figures/flashvsr_ours_comparison.pdf}
    \vspace{-1em}
    \caption{\textbf{Additional visual comparison on VideoLQ dataset.}}
    \label{fig:flashvsr_ours_comparison}
    \vspace{-4mm}
\end{figure}

==> rebuttal/figs/lpips_comparison.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth,height=0.5\columnwidth,keepaspectratio]{rebuttal/figs/figures/lpips_comparison.pdf}
    \vspace{-3em}
    \caption{\textbf{Per-frame LPIPS comparison on REDS4 dataset.}}
    \label{fig:lpips_comparison}
    \vspace{-1.5em}
\end{figure}

==> rebuttal/tables/ablation_with_time_breakdown.tex <==
\begin{table}[t]
\caption{\textbf{Component-wise Runtime \& Quality Analysis}}
\label{tab:rebuttal_breakdown_component}
\centering
\small
\setlength{\tabcolsep}{2pt}  % 欄距壓到最小但可讀
% \renewcommand{\arraystretch}{0.85} % 行距縮小但不重疊
% \vspace{-3mm}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccccccccccc}
\toprule
{Component} & LPIPS$\downarrow$ & DISTS$\downarrow$ & MUSIQ$\uparrow$ & NIQE$\downarrow$ & NRQM$\uparrow$ & BRISQUE$\downarrow$ & tLP$\downarrow$ & tOF$\downarrow$ & WarpErr$\downarrow$ & Time-to-first-frame \\
\midrule
Per-frame & \textcolor{red}{0.099} & 0.071 & \textcolor{blue}{65.981} & 3.249 & 6.969 & 21.655 & 7.261 & 4.201 & 25.668 & \textcolor{red}{0.208} \\
w/o ARTG       & 0.117 & \textcolor{blue}{0.070} & 63.347 & \textcolor{blue}{3.194} & 6.980 & 19.027 & \textcolor{blue}{6.132} & \textcolor{blue}{3.910} & \textcolor{blue}{16.598} & \textcolor{blue}{0.235} \\
w/o TPM        & \textcolor{blue}{0.116} & 0.078 & \textcolor{red}{67.110} & 3.197 & 7.007 & 20.279 & 12.847 & 4.639 & 21.990 & 0.300 \\
TPM (unwarped) & 0.122 & 0.082 & 63.849 & 3.201 & \textcolor{blue}{7.159} & \textcolor{red}{14.063} & 12.846 & 5.689 & 17.143 & 0.320\\
Ours           & \textcolor{red}{0.099} & \textcolor{red}{0.062} & 65.586 & \textcolor{red}{3.111} & \textcolor{red}{7.256} & \textcolor{blue}{17.667} & \textcolor{red}{4.265} & \textcolor{red}{3.620} & \textcolor{red}{14.909} & 0.328 \\
\bottomrule
\end{tabular}%
}
\vspace{-2mm}
\end{table}

==> rebuttal/tables/flashvsr_vs_ours_latency.tex <==
\begin{table}[t]
\caption{\textbf{TTFF comparison on an RTX Pro 6000.}}
\label{tab:flashvsr_ours_latency}

% \vspace{-2mm}
\centering

\scriptsize   % 比 small 更小
\setlength{\tabcolsep}{1.5pt}  % 再縮欄距
\renewcommand{\arraystretch}{0.9} % 壓縮列高

\begin{tabular}{lccc}
\toprule
Method & Chunk Size & Runtime $\downarrow$ & TTFF (ms) $\downarrow$ \\
\midrule
FlashVSR & 6 & 0.283 & 1.698 \\
FlashVSR-Tiny & 6 & \textbf{0.157} & 0.942 \\
Ours & - & 0.243 & \textbf{0.243} \\
\bottomrule
\end{tabular}%

\vspace{-4mm}
\end{table}

==> rebuttal/tables/mix_degradation_comparison.tex <==
\begin{table}[t]
\caption{\textbf{Quantitative comparison on the REDS4 dataset with multi-degradations.}}
\label{tab:mixed_degradation_comparison}
\centering
\small
\setlength{\tabcolsep}{3pt}
% \renewcommand{\arraystretch}{1.1}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llcccccccc}
\toprule
Dir. & Method & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & DISTS$\downarrow$ & MUSIQ$\uparrow$ & tLP$\downarrow$ & tOF$\downarrow$ \\
\midrule
B  & MGLD-VSR & \textcolor{red}{23.305} & \textcolor{blue}{0.594} & \textcolor{blue}{0.246} & \textcolor{blue}{0.112} & 61.139 & 37.737 & 39.039 \\
B  & UAV & 21.721 & 0.534 & 0.419 & 0.22 & 45.714 & \textcolor{blue}{14.687} & 30.589 \\
B  & SeedVR2 & 22.043 & 0.587 & 0.28 & \textcolor{red}{0.111} & 62.213 & 30.273 & \textcolor{red}{14.906} \\
B  & DOVE & \textcolor{blue}{23.128} & \textcolor{red}{0.608} & 0.383 & 0.207 & 52.498 & \textcolor{red}{11.129} & 16.869 \\
\midrule
U  & FlashVSR & 21.163 & 0.527 & 0.287 & 0.124 & \textcolor{red}{63.891} & 14.723 & 24.353 \\
U  & FlashVSR-tiny & 21.462 & 0.536	& 0.307	& 0.142	& 57.593 & 20.221 & 27.106\\
U  & Ours & 22.377 & 0.549 & \textcolor{red}{0.22} & 0.128 & \textcolor{blue}{63.222} & 14.797 & \textcolor{blue}{16.785}\\
\bottomrule
\end{tabular}%
}
\vspace{-4mm}
\end{table}

==> sec/12_only_fig.tex <==
\label{sec:only_fig}


% \FloatBarrier 
% \input{figs/ablation_unet}
% \input{figs/ablation_ART}
% \FloatBarrier

==> tables/ablation/Auto-regressive_temporal_guidance.tex <==
\begin{table*}[htbp]
\caption{\textbf{Ablation study of ARTG.}}
\label{tab:controlnet}
\centering
\vspace{-3mm}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccccccccc}
\toprule
\multirow{2}{*}{Component} & \multicolumn{2}{c}{Reconstruction} & \multicolumn{2}{c}{Reference Perceptual IQA} & \multicolumn{5}{c}{No-reference Perceptual IQA} & \multicolumn{2}{c}{Temporal Consistency} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-10} \cmidrule(lr){11-12}
 & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & DISTS$\downarrow$ & MUSIQ$\uparrow$ & NIQE$\downarrow$ & CLIP-IQA$\uparrow$ & NRQM$\uparrow$ & BRISQUE$\downarrow$ & tLP100$\downarrow$ & tOF$\downarrow$ \\
\midrule
W/O ARTG  & \textcolor{blue}{26.979} & \textcolor{blue}{0.753} & \textcolor{blue}{0.117} & \textcolor{blue}{0.070} & \textcolor{blue}{63.330} & \textcolor{blue}{3.194} & \textcolor{blue}{0.311} & \textcolor{blue}{6.981} & \textcolor{blue}{19.009} & \textcolor{blue}{6.133} & \textcolor{blue}{3.901}\\
Ours     & \textcolor{red}{27.164}  & \textcolor{red}{0.766}  & \textcolor{red}{0.099}  & \textcolor{red}{0.062}  & \textcolor{red}{65.586}  & \textcolor{red}{3.111}  & \textcolor{red}{0.356}  & \textcolor{red}{7.056}  & \textcolor{red}{17.667}  & \textcolor{red}{4.265}  & \textcolor{red}{3.620}\\
\bottomrule
\end{tabular}%
}
\end{table*}


==> tables/ablation/decoder.tex <==
\begin{table*}[t]
\caption{\textbf{Ablation study on the Temporal Processor Module (TPM).} Evaluation of the Temporal Processor Module’s impact on temporal stability. Incorporating TPM improves motion consistency and reduces temporal artifacts, as evidenced by lower tLP100 and tOF scores. The use of warped features further enhances overall video quality.}
\label{tab:decoder}
\centering
\vspace{-3mm}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccccccccc}
\toprule
\multirow{2}{*}{Component} & \multicolumn{2}{c}{Reconstruction} & \multicolumn{2}{c}{Reference Perceptual IQA} & \multicolumn{5}{c}{No-reference Perceptual IQA} & \multicolumn{2}{c}{Temporal Consistency} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-10} \cmidrule(lr){11-12}
 & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & DISTS$\downarrow$ & MUSIQ$\uparrow$ & NIQE$\downarrow$ & CLIP-IQA$\uparrow$ & NRQM$\uparrow$ & BRISQUE$\downarrow$ & tLP100$\downarrow$ & tOF$\downarrow$ \\
\midrule
W/O TPM         & 26.348 & \textcolor{blue}{0.743} & \textcolor{red}{0.099}   & \textcolor{blue}{0.071}   & \textcolor{red}{65.981}  & \textcolor{blue}{3.249}   & \textcolor{red}{0.353}   & 6.969                & 21.655               & \textcolor{blue}{7.261}  & \textcolor{blue}{4.201} \\
TPM (unwarped)  & \textcolor{blue}{26.505} & 0.737 & 0.137                 & 0.089                 & 61.835                & 3.250                & 0.277                 & \textcolor{red}{7.067}  & \textcolor{red}{15.728}  & 16.960               & 5.638 \\
TPM (ours)      & \textcolor{red}{26.979}  & \textcolor{red}{0.753} & \textcolor{blue}{0.117}  & \textcolor{red}{0.070}   & \textcolor{blue}{63.330} & \textcolor{red}{3.194}  & \textcolor{blue}{0.311}  & \textcolor{blue}{6.981}  & \textcolor{blue}{19.009}  & \textcolor{red}{6.133}   & \textcolor{red}{3.901} \\
\bottomrule
\end{tabular}%
}
\end{table*}


==> tables/main/peak_mem.tex <==
\begin{table}[t]
\centering
\small 
\caption{\textbf{Memory and inference speed comparison on NVIDIA A6000.}
OOM = out of memory. Our method achieves the lowest memory footprint, fastest runtime,
and lowest latency.}
\vspace{-3mm}
\label{tab:peak_mem}

\setlength{\tabcolsep}{2pt}  % 欄距壓到最小但可讀
% \renewcommand{\arraystretch}{0.85} % 行距縮小但不重疊
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccc}
\toprule
{Method} & {Peak Memory} & {Per Frame Runtime (s)} & {Latency-max (s)} \\
\midrule
DOVE            & 42.208 GB & 1.74 s & 173.56 s \\
SeedVR2         & OOM & -- & -- \\
Upscale-A-Video & OOM & -- & -- \\
Ours            & \textbf{20.8 GB}     & \textbf{0.67 s}        & \textbf{0.67 s} \\
\bottomrule
\end{tabular}%
}
% \vspace{-4mm}
\end{table}


==> tables/main/table_reds4_bidirectional.tex <==
% \begin{table*}[t]
% \caption{\textbf{Quantitative comparison on the REDS4 dataset.} Quantitative results of various video super-resolution methods on the REDS4 benchmark. Methods are categorized into CNN-based, Transformer-based, and Diffusion-based approaches. Our AR-DiffVSR achieves superior perceptual quality (LPIPS↓) and temporal consistency (tLP100↓, tOF↓) while maintaining significantly lower inference latency compared to other diffusion-based methods. StableVSR* denotes the unidirectional variant of StableVSR.}

% \label{tab:vsr_online_comparison_reds4}
% \centering
% \vspace{-3mm}
% \renewcommand{\arraystretch}{1.1}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lllcccccccccccc}
% \toprule
% Dir. & Method & Conf. & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & DISTS$\downarrow$ & MUSIQ$\uparrow$ & NIQE$\downarrow$ & CLIP-IQA$\uparrow$ & NRQM$\uparrow$ & BRISQUE$\downarrow$ & tLP100$\downarrow$ & tOF$\downarrow$ & Runtime (s)$\downarrow$ \\
% \midrule
% \multicolumn{15}{c}{\textbf{CNN-based Methods}} \\
% \midrule
% -  & Bicubic        & -         & 25.501 & 0.712 & 0.460 & 0.187 & 27.362 & 7.360 & 0.329 & 3.459 & 60.256 & 21.602 & 4.235  & - \\
% B  & BasicVSR++     & CVPR 2022 & 32.391 & 0.907 & 0.131 & 0.069 & 67.013 & 3.851 & 0.381 & 6.366 & 38.637 & 9.017  & 2.49   & 0.098 \\
% B  & RealBasicVSR   & CVPR 2022 & 27.042 & 0.778 & 0.134 & 0.060 & 67.033 & \textcolor{red}{2.530} & 0.372 & 6.769 & 18.046 & 6.421  & 4.754  & \textcolor{blue}{0.064} \\
% U  & TMP            & TIP 2024  & 30.672 & 0.871 & 0.194 & 0.090 & 63.817 & 4.378 & 0.354 & 5.796 & 43.394 & 10.422 & 2.483  & \textcolor{red}{0.041} \\
% \midrule
% \multicolumn{15}{c}{\textbf{Transformer-based Methods}} \\
% \midrule
% B  & RVRT           & NeurIPS 2022 & \textcolor{blue}{32.701} & \textcolor{blue}{0.911} & 0.130 & 0.067 & \textcolor{blue}{67.251} & 3.793 & 0.392 & 6.366 & 38.038 & 9.132  & \textcolor{blue}{2.415} & 0.498 \\
% U  & MIA-VSR        & CVPR 2024    & \textcolor{red}{32.790} & \textcolor{red}{0.912} & 0.123 & 0.064 & \textcolor{red}{68.140} & 3.742 & \textcolor{blue}{0.395} & 6.451 & 37.099 & 8.869  & \textcolor{red}{2.348} & 0.768 \\
% U  & RealViformer   & ECCV 2024    & 26.763 & 0.761 & 0.129 & 0.065 & 64.585 & 2.731 & 0.356 & \textcolor{red}{7.100} & 17.272 & 11.260 & 4.030  & 0.099 \\
% \midrule
% \multicolumn{15}{c}{\textbf{Diffusion-based Methods}} \\
% \midrule
% B  & StableVSR      & ECCV 2024    & 27.928 & 0.793 & \textcolor{blue}{0.102} & \textcolor{red}{0.047} & 67.058 & 2.713 & \textcolor{red}{0.409} & 6.960 & 16.249 & \textcolor{blue}{5.756}  & 2.744  & 46.2 \\
% B  & MGLD-VSR       & ECCV 2024    & 26.530 & 0.749 & 0.151 & 0.065 & 66.081 & 2.972 & 0.364 & 6.701 & \textcolor{red}{15.291} & 18.138 & 5.924  & 43.6 \\
% U  & StableVSR*     & -           & 27.474 & 0.777 & 0.111 & \textcolor{blue}{0.051} & 66.428 & \textcolor{blue}{2.572} & 0.395 & 6.944 & \textcolor{blue}{15.805} & 11.108 & 2.913  & 46.2 \\
% U  & Ours           & -           & 27.164 & 0.766 & \textcolor{red}{0.099} & 0.062 & 65.586 & 3.111 & 0.356 & \textcolor{blue}{7.056} & 17.667 & \textcolor{red}{4.265}  & 3.620  & 0.328 \\
% \bottomrule
% \end{tabular}%
% }
% \end{table*}

\begin{table*}[t]
\caption{
\textbf{Quantitative comparison against bidirectional/offline methods on the REDS4 dataset.} 
We compare CNN-, Transformer-, and diffusion-based methods on REDS4. Stream-DiffVSR achieves superior perceptual and temporal quality with high stability across sequences. \(\uparrow\) indicates higher is better; \(\downarrow\) indicates lower is better. \textbf{Dir.} denotes temporal direction: \textbf{B} for bidirectional/offline, \textbf{U} for unidirectional/online. Runtime is measured per 720p frame on an RTX 4090. \hl{\textbf{TTFF} (time-to-first-frame) denotes the wait between the first input frame and the first output frame, measured over 100-frame video sequences; for offline/bidirectional methods this scales with sequence length, providing a fair end-to-end comparison.} \textbf{tLP} and \textbf{tOF} are scaled by 100× and 10×. Best and second-best results are marked in \textcolor{red}{red} and \textcolor{blue}{blue}.
}

\label{tab:vsr_online_comparison_reds4_bidirectional}
\vspace{-3mm}
\centering
\small
\setlength{\tabcolsep}{3pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llcccccccccccc}
\toprule
Dir. & Method & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & DISTS$\downarrow$ & NIQE$\downarrow$ & NRQM$\uparrow$ & BRISQUE$\downarrow$ & VMAF$\uparrow$ & tLP$\downarrow$ & tOF$\downarrow$ & Runtime (s)$\downarrow$ & \colorbox{yellow}{TTFF} (s)$\downarrow$\\
\midrule
\multicolumn{14}{c}{\textbf{CNN-based Methods}} \\
\midrule
-  & Bicubic & 25.501 & 0.712 & 0.460 & 0.187 & 7.360 & 3.459 & 60.256 & 46.132 & 21.603 & 4.241 & - & - \\
B  & BasicVSR++ & 32.386 & 0.907 & 0.132 & 0.069 & 3.850 & 6.363 & 38.641 & 99.580 & 9.017 & 2.490 & \textcolor{blue}{0.098} & 9.8 \\
B  & RealBasicVSR & 27.042 & 0.778 & 0.134 & 0.065 & \textcolor{red}{2.530} & 6.769 & 18.046 & 88.197 & 6.422 & 4.759 & \textcolor{red}{0.064} & \textcolor{blue}{6.4} \\
\midrule
\multicolumn{14}{c}{\textbf{Transformer-based Methods}} \\
\midrule
B  & RVRT & \textcolor{blue}{32.701} & \textcolor{blue}{0.911} & 0.130 & 0.067 & 3.793 & 6.366 & 38.038 & \textcolor{red}{99.681} & 9.133 & \textcolor{blue}{2.421} & 0.498 & 2.49 \\
B  & MIA-VSR & \textcolor{red}{32.790} & \textcolor{red}{0.912} & 0.123 & 0.064 & \textcolor{blue}{3.742} & 6.451 & 37.099 & \textcolor{blue}{99.669} & 8.870 & \textcolor{red}{2.354} & 0.768 & 76.8 \\
\midrule
\multicolumn{14}{c}{\textbf{Diffusion-based Methods}} \\
\midrule
B  & StableVSR & 27.928 & 0.793 & \textcolor{blue}{0.102} & \textcolor{red}{0.047} & \textcolor{red}{2.713} & \textcolor{blue}{6.960} & \textcolor{blue}{16.249} & 95.303 & \textcolor{blue}{5.755} & 2.742 & 46.2 & 4620 \\
B  & MGLD-VSR & 26.53 & 0.749 & 0.151 & 0.065 & 2.972 & 6.701 & \textcolor{red}{15.291} & 78.255 & 18.139 & 5.910 & 43.6 & 218 \\
U  & Ours & 27.256 & 0.766 & \textcolor{red}{0.099} & \textcolor{blue}{0.062} & 3.114 & \textcolor{red}{7.055} & 17.717 & 88.751 & \textcolor{red}{4.198} & 3.638 & 0.328 & \textcolor{red}{0.328} \\
\bottomrule
\end{tabular}%
}
\end{table*}

==> tables/main/table_reds4_dit.tex <==
\begin{table*}[t]
% \caption{
% \textbf{Quantitative comparison on the REDS4 dataset.} We evaluate the performance of various video super-resolution methods, including CNN-, Transformer-, and diffusion-based approaches on the REDS4 benchmark. Our AR-DiffVSR achieves superior perceptual quality and temporal consistency, while also demonstrating high output stability across different video sequences. All results are reported as \textit{mean ± standard deviation} across the 4 videos in the REDS4 dataset. Arrows in column headers indicate the direction of improvement: \(\uparrow\) means higher is better, \(\downarrow\) means lower is better. \textbf{Dir.} indicates the temporal direction used for each method: \textbf{B} for bidirectional/offline and \textbf{U} for unidirectional/online (past-only) models. Runtime denotes the average per-frame inference time (in seconds) on 720p videos using a single NVIDIA RTX 4090 GPU. Results are measured using the official implementations where available. Note: for readability, \textbf{tLP100 is scaled by 100×}, \textbf{tOF by 10×}, and \textbf{WarpErr by 1000×}. Best and second-best results are highlighted in \textcolor{red}{red} and \textcolor{blue}{blue}, respectively.}
\caption{
\textbf{Quantitative comparison against DiT methods on the REDS4 dataset.} Runtime is measured on an RTX Pro 6000.\textcolor{gray}{Gray-shaded entries are reported from FlashVSR}; “--” indicates unavailable results.}
\label{tab:vsr_online_comparison_reds4_dit}
\vspace{-3mm}
\centering
\small
\setlength{\tabcolsep}{3pt}
% \renewcommand{\arraystretch}{1.1}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llccccccccccccccc}
\toprule
Dir. & Method & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & DISTS$\downarrow$ & MUSIQ$\uparrow$ & NIQE$\downarrow$ & NRQM$\uparrow$ & BRISQUE$\downarrow$ & VMAF$\uparrow$ & tLP$\downarrow$ & tOF$\downarrow$ & Runtime (s)$\downarrow$ & \colorbox{yellow}{TTFF} (s)$\downarrow$ & Peak Mem (GB)\\
\midrule
B  & UAV & 23.077 & 0.608 & 0.495 & 0.249 & 30.912 & 5.917 & 3.666 & 39.751 & 20.600 & 30.546 & 13.582 & 6.017 & 601.740 & 57.094 \\
\rowcolor{black!10}
B  & UAV & 24.840 & 0.644 & 0.41 & -- & 53.000 & 3.104 & -- & -- & -- & -- & -- & -- & -- & -- \\
B  & SeedVR2 & 22.774 & 0.661 & \textcolor{blue}{0.246} & \textcolor{blue}{0.111} & \textcolor{blue}{65.011} & \textcolor{red}{2.812} & \textcolor{blue}{6.707} & 29.948 & \textcolor{blue}{64.447} & 30.296 & 12.79 & 0.479 & 47.840 & 69.592 \\
\rowcolor{black!10}
B  & SeedVR2 & 24.830 & 0.704 & 0.312 & -- & 61.830 & 3.066 & -- & -- & -- & -- & -- & -- & -- & -- \\
B  & DOVE & \textcolor{blue}{25.027} & \textcolor{blue}{0.692} & 0.291 & 0.149 & 54.060 & 4.087 & 5.753 & 25.606 & 58.329 & \textcolor{blue}{10.260} & \textcolor{blue}{10.960} & 0.760 & 75.983 & 42.208 \\
B  & VEnhancer & 20.712 & 0.560 & 0.384 & 0.156 & 56.932 & 4.142 & 5.567 & \textcolor{blue}{24.906} & 24.743 & 32.913 & 16.643 & 0.672 & 671.650 & 53.200 \\
U  & FlashVSR & 21.484 & 0.569 & 0.283 & 0.124 & 62.178 & 6.574 & 6.574 & 25.821 & 40.556 & 15.69 & 20.548 & 0.283 & 1.698 & 19.630 \\
\rowcolor{black!10}
U  & FlashVSR & 23.920 & 0.649 & 0.343 & 0.124 & 68.97 & 2.425 & 6.574 & 25.821 & 40.556 & 15.69 & 20.548 & 0.283 & 1.698 & 19.630 \\
U  & FlashVSR-tiny & 21.887 & 0.577 & 0.300 & 0.141 & 55.204 & 3.463 & 6.188 & 28.589 & 38.634 & 17.838 & 23.992 & \textcolor{red}{0.157} & \textcolor{blue}{0.942} & \textcolor{red}{12.390} \\
\rowcolor{black!10}
U  & FlashVSR-tiny & 24.110 & 0.651 & 0.343 & -- & 67.43 & 2.680 & -- & -- & -- & -- & -- & -- & -- & -- \\
U  & Ours & \textcolor{red}{27.256} & \textcolor{red}{0.766} & \textcolor{red}{0.098} & \textcolor{red}{0.062} & \textcolor{red}{65.595} & \textcolor{blue}{3.111} & \textcolor{red}{7.056} & \textcolor{red}{17.667} & \textcolor{red}{88.751} & \textcolor{red}{4.198} & \textcolor{red}{3.638} & \textcolor{blue}{0.243} & \textcolor{red}{0.243} & \textcolor{blue}{19.580}\\
\bottomrule
\end{tabular}%
}
% \vspace{-2mm}
\end{table*}

==> tables/main/table_reds4_unidirectional.tex <==
\begin{table*}[t]
% \caption{
% \textbf{Quantitative comparison on the REDS4 dataset.} We evaluate the performance of various video super-resolution methods, including CNN-, Transformer-, and diffusion-based approaches on the REDS4 benchmark. Our AR-DiffVSR achieves superior perceptual quality and temporal consistency, while also demonstrating high output stability across different video sequences. All results are reported as \textit{mean ± standard deviation} across the 4 videos in the REDS4 dataset. Arrows in column headers indicate the direction of improvement: \(\uparrow\) means higher is better, \(\downarrow\) means lower is better. \textbf{Dir.} indicates the temporal direction used for each method: \textbf{B} for bidirectional/offline and \textbf{U} for unidirectional/online (past-only) models. Runtime denotes the average per-frame inference time (in seconds) on 720p videos using a single NVIDIA RTX 4090 GPU. Results are measured using the official implementations where available. Note: for readability, \textbf{tLP100 is scaled by 100×}, \textbf{tOF by 10×}, and \textbf{WarpErr by 1000×}. Best and second-best results are highlighted in \textcolor{red}{red} and \textcolor{blue}{blue}, respectively.}
\caption{
\textbf{Quantitative comparison against unidirectional/online methods on the REDS4 dataset.}}
\label{tab:vsr_online_comparison_reds4_unidirectional}
\vspace{-3mm}
\centering
\small
\setlength{\tabcolsep}{3pt}
% \renewcommand{\arraystretch}{1.1}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llcccccccccccccc}
\toprule
Dir. & Method & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & DISTS$\downarrow$ & MUSIQ$\uparrow$ & NIQE$\downarrow$ & NRQM$\uparrow$ & BRISQUE$\downarrow$ & VMAF$\uparrow$ & tLP$\downarrow$ & tOF$\downarrow$ & Runtime (s)$\downarrow$ & \colorbox{yellow}{TTFF} (s)$\downarrow$\\
\midrule
\multicolumn{15}{c}{\textbf{CNN-based Methods}} \\
\midrule
-  & Bicubic & 25.501 & 0.712 & 0.460 & 0.187 & 27.362 & 7.360 & 3.459 & 60.256 & 46.132 & 21.603 & 4.241 & - & - \\
U  & TMP & \textcolor{red}{30.672} & \textcolor{red}{0.871} & 0.194 & 0.090 & 63.818 & 4.378 & 5.796 & 43.394 & \textcolor{red}{98.586} & 10.424 & \textcolor{red}{2.480} & \textcolor{red}{0.041} & \textcolor{red}{0.041} \\
\midrule
\multicolumn{15}{c}{\textbf{Transformer-based Methods}} \\
\midrule
U  & RealViformer & 26.763 & 0.761 & 0.129 & 0.065 & 64.585 & \textcolor{blue}{2.731} & \textcolor{blue}{7.028} & 17.272 & 60.509 & 11.261 & 4.037 & \textcolor{blue}{0.099} & 9.9 \\
\midrule
\multicolumn{15}{c}{\textbf{Diffusion-based Methods}} \\
\midrule
U  & StableVSR* & 27.174 & 0.763 & \textcolor{blue}{0.111} & \textcolor{red}{0.051} & \textcolor{red}{66.428} & \textcolor{red}{2.572} & 6.944 & \textcolor{red}{15.805} & 88.675 & 11.107 & 3.925 & 46.2 & 4620 \\
U  & Ours & \textcolor{blue}{27.256} & \textcolor{blue}{0.766} & \textcolor{red}{0.099} & \textcolor{blue}{0.062} & \textcolor{blue}{65.595} & 3.114 & \textcolor{red}{7.055} & \textcolor{blue}{17.117} & \textcolor{blue}{88.751} & \textcolor{red}{4.198} & \textcolor{blue}{3.638} & 0.328 & \textcolor{blue}{0.328} \\
\bottomrule
\end{tabular}%
}
% \vspace{-2mm}
\end{table*}

==> tables/main/table_udm10.tex <==
\begin{table*}[t]
\caption{\textbf{Quantitative comparison on the UDM10 dataset.} Best and second-best results are highlighted in \textcolor{red}{red} and \textcolor{blue}{blue}, respectively.}
\label{tab:vsr_online_comparison_udm10}
\vspace{-4mm}
\centering
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.1}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llccccccccc}
\toprule
Dir.\ & Method            & LPIPS $\downarrow$ & DISTS $\downarrow$ & MUSIQ $\uparrow$ & CLIP-IQA $\uparrow$ & tLP $\downarrow$ & tOF $\downarrow$ & WarpErr $\downarrow$ & Runtime(s) $\downarrow$\\
\midrule
\multicolumn{10}{c}{\textbf{CNN-based Methods}} \\
\midrule
- & Bicubic           & - & - & - & - &  & $4.241\pm5.765$  & $4.371\pm1.861$    & - \\
B & BasicVSR++        & $0.132\pm0.023$  & $0.069\pm0.012$  & $67.002\pm4.291$    & $0.381\pm0.074$    & $9.017\pm4.384$  & $2.490\pm4.440$  & $6.998\pm2.376$    & 0.098 \\
B & RealBasicVSR      & $0.134\pm0.016$  & $0.060\pm0.006$  & $67.033\pm4.283$    & $0.372\pm0.084$    & $6.422\pm4.726$  & $4.759\pm7.722$  & $13.256\pm4.559$   & 0.064 \\
U & TMP               & $0.194\pm0.039$  & $0.090\pm0.010$  & $63.818\pm4.129$    & $0.354\pm0.071$    & $10.424\pm5.654$  & $2.480\pm3.852$  & $6.814\pm2.426$    & 0.041 \\
\midrule
\multicolumn{10}{c}{\textbf{Transformer-based Methods}} \\
\midrule
B & RVRT              & $0.130\pm0.022$  & $0.067\pm0.011$  & $67.251\pm4.372$    & $0.392\pm0.072$    & $9.133\pm4.408$  & $2.421\pm4.316$  & $7.148\pm2.409$    & 0.498 \\
U & MIA-VSR           & $0.123\pm0.022$  & $0.064\pm0.011$  & $68.140\pm3.964$    & $0.395\pm0.067$    & $8.870\pm4.606$  & $2.354\pm4.026$  & $7.188\pm2.433$    & 0.768 \\
U & RealViformer      & $0.129\pm0.015$  & $0.065\pm0.004$  & $64.585\pm5.117$    & $0.356\pm0.079$    & $11.261\pm5.755$  & $4.037\pm5.613$  & $11.782\pm3.762$   & 0.099 \\
\midrule
\multicolumn{10}{c}{\textbf{Diffusion-based Methods}} \\
\midrule
B & StableVSR         & $0.102\pm0.015$  & $0.047\pm0.006$  & $67.058\pm3.797$    & $0.409\pm0.089$    & $5.755\pm4.618$  & $2.742\pm4.741$  & $14.970\pm5.843$   & 46.2 \\
B & MGLD-VSR          & $0.151\pm0.019$  & $0.065\pm0.006$  & $66.081\pm4.027$    & $0.364\pm0.077$    & $18.139\pm8.772$  & $5.910\pm6.888$  & $15.118\pm5.156$   & 43.6 \\
U & StableVSR*        & $0.111\pm0.017$  & $0.051\pm0.006$  & $66.428\pm4.040$    & $0.395\pm0.091$    & $11.107\pm8.293$  & $2.925\pm4.561$  & $17.644\pm7.266$   & 46.2 \\
U & Ours              & $-\pm-$  & $-\pm-$  & $-\pm-$    & $-\pm-$    & $-\pm-$  & $-\pm-$  & $-\pm-$   & 0.328\\
\bottomrule
\end{tabular}%
}
\end{table*}


==> tables/main/table_vid4_bidirectional.tex <==
% \begin{table*}[t]
% \caption{\textbf{Quantitative comparisons of different VSR methods on the Vid4 dataset.} Best and second-best results are highlighted in \textcolor{red}{red} and \textcolor{blue}{blue}, respectively.}
% \label{tab:vsr_online_comparison}
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l l c c c c c c c c c c c c c}
% \toprule
% \multirow{2}{*}{{Type}} 
% & \multirow{2}{*}{Method} 
% & \multirow{2}{*}{Conference}
% & \multicolumn{2}{c}{Reconstruction} 
% & \multicolumn{2}{c}{Reference Perceptual IQA}
% & \multicolumn{5}{c}{No-reference Perceptual IQA}
% & \multicolumn{2}{c}{Temporal Consistency}
% & \multirow{2}{*}{Runtime (s)} \\
% \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-12} \cmidrule(lr){13-14}
% & & 
% & PSNR$\uparrow$ & SSIM$\uparrow$
% & LPIPS$\downarrow$ & DISTS$\downarrow$
% & MUSIQ$\uparrow$ & NIQE$\downarrow$ & CLIP-IQA$\uparrow$ & NRQM$\uparrow$
% & BRISQUE$\downarrow$ & tLP100$\downarrow$ & tOF$\downarrow$
% & \\
% \midrule
% % ------------------ (1) Bidirectional group ------------------
% \multirow{6}{*}{\rotatebox[origin=c]{90}{Bidirectional}}
% & Bicubic & -
%   & 21.719 & 0.582
%   & 0.516 & 0.216
%   & 26.666 & 7.738 & 0.349 & 3.463
%   & 58.705 & 27.278
%   & 1.124
%   & - \\
% & StableVSR & ECCV 2024
%   & 22.541 & 0.644
%   & 0.199 & 0.103
%   & 67.362 & 2.569 & 0.492 & 7.310
%   & 12.716 & 48.765
%   & 0.926 & - \\
% & MGLD-VSR & ECCV 2024
%   & 21.983 & 0.605 & 0.246 & 0.139 & 66.479 & 3.092 & 0.405 & 7.185 & 16.420 & 31.776 & 3.235 & - \\
% & RVRT & NeurIPS 2022
%   & 26.377 & 0.826 & 0.227 & 0.129 & 57.894 & 5.171 & 0.335 & 6.134 & 44.659 & 16.970 & 0.490 & - \\
% & BasicVSR++ & CVPR 2022
%   & 26.230 & 0.828 & 0.190 & 0.122 & 61.497 & 5.044 & 0.341 & 6.589 & 38.108 & 15.055 & 0.488 & - \\
% & RealBasicVSR & CVPR 2022
%   & 22.823 & 0.662 & 0.214 & 0.122 & 67.275 & 2.950 & 0.371 & 7.202 & 22.366 & 6.812 & 0.866 \\
% \midrule
% % ------------------ (2) Unidirectional group ------------------
% \multirow{5}{*}{\rotatebox[origin=c]{90}{Unidirectional}}
% & StableVSR* & -
%   & 22.213 & 0.623 & 0.208 & 0.105 & 67.395 & 2.536 & 0.489 & 7.319 & 11.335 & 60.150 & 1.009 \\
% & MIA-VSR & CVPR 2024
%   & 26.175 & 0.826 & 0.175 & 0.120 & 63.597 & 4.554 & 0.369 & 6.714 & 38.441 & 14.358 & 0.488 \\
% & TMP  & TIP 2024
%   & 25.579 & 0.797 & 0.254 & 0.141 & 56.389 & 5.488 & 0.299 & 5.839 & 46.526 & 14.086 & 0.547 \\
% & RealViformer & ECCV 2024
%   & 21.963 & 0.597 & 0.256 & 0.150 & 63.059 & 3.671 & 0.328 & 7.580 & 20.695 & 11.658 & 1.055 \\
% & Ours & -
%   & 22.725 & 0.652 & 0.199 & 0.132 & 63.911 & 3.511 & 0.292 & 7.223 & 22.581
%   & 13.984 & 1.032
%   & - \\

% \bottomrule
% \end{tabular}
% }
% \end{table*}

\begin{table*}[t]
% \vspace{-3mm}
\caption{\textbf{Quantitative comparison against bidirectional/offline methods on the Vid4 dataset.} 
% We evaluate the no-reference quality of various VSR methods on the VideoLQ benchmark. Best and second-best results are highlighted in \textcolor{red}{red} and \textcolor{blue}{blue}, respectively.
}
\label{tab:vsr_online_comparison_vid4_bidirectional}
\vspace{-3mm}
\small
\centering
% \setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{0.8}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llcccccccc}
\toprule
Dir. & Method & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & NRQM$\uparrow$ & BRISQUE$\downarrow$ & tLP$\downarrow$ & tOF$\downarrow$ & latency-max (s)$\downarrow$\\
\midrule
\multicolumn{10}{c}{\textbf{CNN-based Methods}} \\
\midrule
- & Bicubic        & 21.719 & 0.582 & 0.512 & 3.429 & 58.680 & 27.819 & 1.145 & - \\
B & BasicVSR++     & \textcolor{red}{26.230} & \textcolor{blue}{0.828} & 0.193 & 6.481 & 38.409 & 15.029 &  \textcolor{blue}{0.507} & 6.86 \\
B & RealBasicVSR   & 21.963 & 0.597 & 0.210 & 7.122 & 21.804 &  \textcolor{red}{6.630} & 0.9 & \textcolor{blue}{4.48} \\
\midrule
\multicolumn{10}{c}{\textbf{Transformer-based Methods}} \\
\midrule
B & RVRT           & \textcolor{red}{26.377} & \textcolor{blue}{0.826} & 0.229 & 6.006 & 44.667 & 17.146 &  \textcolor{blue}{0.507} & 1.743 \\
B & MIA-VSR        & 26.175 & \textcolor{blue}{0.826} & \textcolor{red}{0.174} & 6.619 & 38.509 & 14.297 &  \textcolor{red}{0.505} & 53.76 \\
\midrule
\multicolumn{10}{c}{\textbf{Diffusion-based Methods}} \\
\midrule
B & StableVSR      & 22.541 & 0.644 & 0.194 & \textcolor{blue}{7.224} &  \textcolor{blue}{13.254} & 48.585 & 0.957 & 3234 \\
B & MGLD-VSR       & 21.983 & 0.605 & 0.243 & 7.129 & 16.525 & 31.744 & 3.152 & 152.6 \\
\midrule
U & Ours           & 22.725 & 0.652 &  \textcolor{blue}{0.191} &  \textcolor{red}{7.346} & \textcolor{blue}{15.260} &  \textcolor{blue}{8.985} & 0.962 & \textcolor{red}{0.229} \\
\bottomrule
\end{tabular}%
}
\vspace{-3mm}
\end{table*}

==> tables/main/table_vid4_unidirectional.tex <==
\begin{table*}[t]
% \vspace{-2mm}
\caption{\textbf{Quantitative comparison against unidirectional/online methods on the Vid4 dataset.}}
\label{tab:vid4_unidirectional}
\vspace{-3mm}
\centering
\small
% \setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{0.8}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llcccccccc}
\toprule
Dir. & Method & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & NRQM$\uparrow$ & BRISQUE$\downarrow$ & tLP$\downarrow$ & tOF$\downarrow$ & latency-max (s)$\downarrow$ \\
\midrule
\multicolumn{10}{c}{\textbf{CNN-based Methods}} \\
\midrule
- & Bicubic        & 21.719 & 0.582 & 0.512 & 3.429 & 58.680 & 27.819 & 1.145 & - \\
U & TMP            & \textcolor{red}{25.579} & \textcolor{red}{0.797} & 0.256 & 5.698 & 46.257 & 14.199 & \textcolor{red}{0.566} & \textcolor{red}{0.029} \\
\midrule
\multicolumn{10}{c}{\textbf{Transformer-based Methods}} \\
\midrule
U & RealViformer   & 21.963 & 0.597 & 0.257 &  \textcolor{red}{7.604} & 21.804 & \textcolor{blue}{11.633} & 1.107 & 6.93 \\
\midrule
\multicolumn{10}{c}{\textbf{Diffusion-based Methods}} \\
\midrule
U & StableVSR*     & 22.213 & 0.623 & \textcolor{blue}{0.203} & 7.233 &  \textcolor{red}{11.966} & 59.594 & 1.036 & 3234 \\
\midrule
U & Ours           & \textcolor{blue}{22.725} & \textcolor{blue}{0.652} &  \textcolor{red}{0.191} &  \textcolor{blue}{7.346} & \textcolor{blue}{15.260} &  \textcolor{blue}{8.985} & \textcolor{blue}{0.962} & \textcolor{blue}{0.229} \\
\bottomrule
\end{tabular}%
}
\vspace{-3mm}
\end{table*}

==> tables/main/table_videoLQ_bidirectional.tex <==
% \begin{table}[t]
% \caption{\textbf{Quantitative comparison on the VideoLQ dataset.} We evaluate the perceptual and no-reference quality of various VSR methods on the VideoLQ benchmark. All results are reported as \textit{mean ± standard deviation}. Arrows in column headers indicate the direction of improvement: \(\uparrow\) means higher is better, \(\downarrow\) means lower is better. \textbf{Dir.} indicates the temporal direction used for each method: \textbf{B} for bidirectional/offline and \textbf{U} for unidirectional/online (past-only) models. Best and second-best results are highlighted in \textcolor{red}{red} and \textcolor{blue}{blue}, respectively.}
% \label{tab:vsr_online_comparison_videolq}
% \centering
% \small
% \setlength{\tabcolsep}{2pt}
% \renewcommand{\arraystretch}{1.1}
% % \resizebox{\textwidth}{!}{%
% \begin{tabular}{llccccc}
% \toprule
% Dir. & Method & MUSIQ$\uparrow$ & NIQE$\downarrow$ & CLIP-IQA$\uparrow$ & NRQM$\uparrow$ & BRISQUE$\downarrow$ \\
% \midrule
% \multicolumn{7}{c}{\textbf{CNN-based Methods}} \\
% \midrule
% - & Bicubic        & $25.151 \pm 6.545$& $7.945 \pm 0.608$ & $0.306 \pm 0.060$ & $3.151 \pm 0.302$ & $57.944 \pm 4.490$ \\
% B & BasicVSR++     & $32.659 \pm 9.690$ & $5.909 \pm 0.979$ & $0.281 \pm 0.084$ & $3.745 \pm 0.822$ & $56.800 \pm 8.602$ \\
% B & RealBasicVSR   & $56.779 \pm 8.145$ & $3.973 \pm 0.622$ & $0.367 \pm 0.127$ & $6.095 \pm 0.403$ & $30.158 \pm 10.464$ \\
% U & TMP            & $32.431 \pm 10.133$ & $6.751 \pm 0.601$ & $0.266 \pm 0.078$ & $3.511 \pm 0.590$ & $59.841 \pm 6.308$ \\
% \midrule
% \multicolumn{7}{c}{\textbf{Transformer-based Methods}} \\
% \midrule
% B & RVRT           & $31.136 \pm 9.667$ & $6.939 \pm 0.674$ & $0.279 \pm 0.085$ & $3.493 \pm 0.528$ & $60.557 \pm 6.046$ \\
% U & MIA-VSR        & $33.006 \pm 10.946$ & $5.860 \pm 1.065$ & $0.255 \pm 0.080$ & $3.810 \pm 0.865$ & $58.513 \pm 6.959$ \\
% B & RealViformer   & $51.988 \pm 8.591$ & $4.070 \pm 0.814$ & $0.344 \pm 0.120$ & $6.066 \pm 0.969$ & $28.266 \pm 7.420$ \\
% \midrule
% \multicolumn{7}{c}{\textbf{Diffusion-based Methods}} \\
% \midrule
% B & StableVSR      & $35.262 \pm 13.391$ & $3.973 \pm 0.745$ & $0.268 \pm 0.128$ & $6.154 \pm 1.117$ & $22.973 \pm 8.831$ \\
% B & MGLD-VSR       & $51.896 \pm 9.340$ & $4.163 \pm 1.003$ & $0.338 \pm 0.113$ & $5.761 \pm 0.924$ & $29.497 \pm 6.876$ \\
% U & StableVSR*     & $35.462 \pm 13.232$ & $3.982 \pm 0.741$ & $0.266 \pm 0.124$ & $6.122 \pm 1.167$ & $23.814 \pm 8.450$ \\
% \midrule
% U & Ours           & $40.371 \pm 15.127$ & $4.162 \pm 0.64$ & $0.259 \pm 0.103$ & $6.04 \pm 1.086$ & $27.176 \pm 5.664$ \\
% \bottomrule
% \end{tabular}%
% % }
% \end{table}

% \begin{table}[t]
% \tiny
% \renewcommand{\arraystretch}{0.85}
% \vspace{-3mm}
% \centering
% \caption{\textbf{Quantitative comparison against bidirectional/offline methods on the VideoLQ dataset.}}
% % We evaluate the no-reference quality of various VSR methods on the VideoLQ benchmark. Best and second-best results are highlighted in \textcolor{red}{red} and \textcolor{blue}{blue}, respectively.}
% \label{tab:vsr_online_comparison_videolq_bidirectional}
% \vspace{-3mm}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{llccc}
% \toprule
% Dir. & Method & NIQE$\downarrow$ & NRQM$\uparrow$ & BRISQUE$\downarrow$ \\
% \midrule
% \multicolumn{5}{c}{\textbf{CNN-based Methods}} \\
% \midrule
% - & Bicubic        & 7.945 & 3.151 & 57.944 \\
% B & BasicVSR++     & 5.909 & 3.745 & 56.800 \\
% B & RealBasicVSR   & \textcolor{blue}{3.973} & 6.095 & 30.158 \\
% \midrule
% \multicolumn{5}{c}{\textbf{Transformer-based Methods}} \\
% \midrule
% B & RVRT           & 6.939 & 3.493 & 60.557 \\
% B & MIA-VSR        & 5.860 & 3.810 & 58.513 \\
% \midrule
% \multicolumn{5}{c}{\textbf{Diffusion-based Methods}} \\
% \midrule
% B & StableVSR      & \textcolor{blue}{3.973} &  \textcolor{red}{6.154} &  \textcolor{red}{22.973} \\
% B & MGLD-VSR       & 4.163 & 5.761 & 29.497 \\
% \midrule
% U & Ours           & \textcolor{red}{3.929} &  \textcolor{blue}{6.140} &  \textcolor{blue}{23.176} \\
% \bottomrule
% \end{tabular}%
% }
% \end{table}
% \vspace{-3mm}
% \begin{table}[t]
% \tiny
% \renewcommand{\arraystretch}{0.85}
% \vspace{-3mm}
% \centering
% \caption{\textbf{Quantitative comparison against unidirectional/online methods on the VideoLQ dataset.} 
% % We evaluate the no-reference quality of various VSR methods on the VideoLQ benchmark. Best and second-best results are highlighted in \textcolor{red}{red} and \textcolor{blue}{blue}, respectively.
% }
% \label{tab:vsr_online_comparison_videolq_unidirectional}
% \vspace{-3mm}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{llccc}
% \toprule
% Dir. & Method & NIQE$\downarrow$ & NRQM$\uparrow$ & BRISQUE$\downarrow$ \\
% \midrule
% \multicolumn{5}{c}{\textbf{CNN-based Methods}} \\
% \midrule
% - & Bicubic        & 7.945 & 3.151 & 57.944 \\
% U & TMP            & 6.751 & 3.511 & 59.841 \\
% \midrule
% \multicolumn{5}{c}{\textbf{Transformer-based Methods}} \\
% \midrule
% U & RealViformer   & 4.070 & 6.066 & 28.266 \\
% \midrule
% \multicolumn{5}{c}{\textbf{Diffusion-based Methods}} \\
% \midrule
% U & StableVSR*     & \textcolor{blue}{3.982} & \textcolor{blue}{6.122} & \textcolor{blue}{23.814} \\
% \midrule
% U & Ours           & \textcolor{red}{3.929} &  \textcolor{red}{6.140} &  \textcolor{red}{23.176} \\
% \bottomrule
% \end{tabular}%
% }
% \end{table}


% \begin{table*}[t]
% \centering
% \tiny
% \renewcommand{\arraystretch}{0.85}
% \vspace{-5mm}
% \caption{\textbf{Quantitative comparison on the VideoLQ dataset.} Left: Against bidirectional/offline methods ; Right: unidirectional/online methods.}
% \label{tab:videoLQ_combined}
% \vspace{-5mm}
% \begin{tabular}{cc}
% % 左表 ============
% \vspace{-4mm}
% \begin{minipage}{.5\textwidth}
% \renewcommand{\arraystretch}{0.5} 
% \small
% \centering
% \caption*{\textbf{(a) Bidirectional/Offline}}
% \vspace{-4mm}
% \begin{tabular}{llccc}
% \toprule
% Dir. & Method & NIQE$\downarrow$ & NRQM$\uparrow$ & BRISQUE$\downarrow$ \\
% \midrule
% \multicolumn{5}{c}{\textbf{CNN-based Methods}} \\
% \midrule
% - & Bicubic        & 7.945 & 3.151 & 57.944 \\
% B & BasicVSR++     & 5.909 & 3.745 & 56.800 \\
% B & RealBasicVSR   & \textcolor{blue}{3.973} & 6.095 & 30.158 \\
% \midrule
% \multicolumn{5}{c}{\textbf{Transformer-based Methods}} \\
% \midrule
% B & RVRT           & 6.939 & 3.493 & 60.557 \\
% B & MIA-VSR        & 5.860 & 3.810 & 58.513 \\
% \midrule
% \multicolumn{5}{c}{\textbf{Diffusion-based Methods}} \\
% \midrule
% B & StableVSR      & \textcolor{blue}{3.973} &  \textcolor{red}{6.154} &  \textcolor{red}{22.973} \\
% B & MGLD-VSR       & 4.163 & 5.761 & 29.497 \\
% \midrule
% U & Ours           & \textcolor{red}{3.929} &  \textcolor{blue}{6.140} &  \textcolor{blue}{23.176} \\
% \bottomrule
% \end{tabular}
% \end{minipage}
% &
% % 右表 ============
% \vspace{-4mm}
% \begin{minipage}{.5\textwidth}
% \small
% \centering
% \caption*{\textbf{(b) Unidirectional/Online}}
% \vspace{-4mm}
% \begin{tabular}{llccc}
% \toprule
% Dir. & Method & NIQE$\downarrow$ & NRQM$\uparrow$ & BRISQUE$\downarrow$ \\
% \midrule
% \multicolumn{5}{c}{\textbf{CNN-based Methods}} \\
% \midrule
% - & Bicubic        & 7.945 & 3.151 & 57.944 \\
% U & TMP            & 6.751 & 3.511 & 59.841 \\
% \midrule
% \multicolumn{5}{c}{\textbf{Transformer-based Methods}} \\
% \midrule
% U & RealViformer   & 4.070 & 6.066 & 28.266 \\
% \midrule
% \multicolumn{5}{c}{\textbf{Diffusion-based Methods}} \\
% \midrule
% U & StableVSR*     & \textcolor{blue}{3.982} & \textcolor{blue}{6.122} & \textcolor{blue}{23.814} \\
% \midrule
% U & Ours           & \textcolor{red}{3.929} &  \textcolor{red}{6.140} &  \textcolor{red}{23.176} \\
% \bottomrule
% \end{tabular}
% \end{minipage}
% \\  % row end
% \end{tabular}
% \vspace{6mm}
% \end{table*}

\begin{table*}[t]
\centering
% \caption{\textbf{Quantitative comparison on the VideoLQ dataset.} Left: bidirectional/offline methods; Right: unidirectional/online methods.}
\caption{\textbf{Quantitative comparison on the VideoLQ dataset.}}
\label{tab:videoLQ_combined}
\vspace{-6mm}
% 建議：不要大量負 vspace，先靠 col/row spacing 控制
\setlength{\tabcolsep}{3pt}      % 縮欄距（可 2.5pt~4pt 試）
\renewcommand{\arraystretch}{0.9}
\begin{minipage}[t]{0.47\textwidth}
\centering
\caption*{\textbf{(a) Bidirectional/Offline}}
\vspace{-3mm}
\resizebox{\linewidth}{!}{%
\begin{tabular}{llccc}
\toprule
Dir. & Method & NIQE$\downarrow$ & NRQM$\uparrow$ & BRISQUE$\downarrow$ \\
\midrule
\multicolumn{5}{c}{\textbf{CNN-based Methods}} \\
\midrule
- & Bicubic        & 7.945 & 3.151 & 57.944 \\
B & BasicVSR++     & 5.909 & 3.745 & 56.800 \\
B & RealBasicVSR   & \textcolor{blue}{3.973} & 6.095 & 30.158 \\
\midrule
\multicolumn{5}{c}{\textbf{Transformer-based Methods}} \\
\midrule
B & RVRT           & 6.939 & 3.493 & 60.557 \\
B & MIA-VSR        & 5.860 & 3.810 & 58.513 \\
\midrule
\multicolumn{5}{c}{\textbf{Diffusion-based Methods}} \\
\midrule
B & StableVSR      & \textcolor{blue}{3.973} & \textcolor{red}{6.154} & \textcolor{red}{22.973} \\
B & MGLD-VSR       & 4.163 & 5.761 & 29.497 \\
\midrule
U & Ours           & \textcolor{red}{3.929} & \textcolor{blue}{6.140} & \textcolor{blue}{23.176} \\
\bottomrule
\end{tabular}}
\end{minipage}
\hfill
\begin{minipage}[t]{0.49\textwidth}
\centering
\caption*{\textbf{(b) Unidirectional/Online}}
\vspace{1mm}
\resizebox{\linewidth}{!}{%
\begin{tabular}{llccc}
\toprule
Dir. & Method & NIQE$\downarrow$ & NRQM$\uparrow$ & BRISQUE$\downarrow$ \\
\midrule
\multicolumn{5}{c}{\textbf{CNN-based Methods}} \\
\midrule
- & Bicubic        & 7.945 & 3.151 & 57.944 \\
U & TMP            & 6.751 & 3.511 & 59.841 \\
\midrule
\multicolumn{5}{c}{\textbf{Transformer-based Methods}} \\
\midrule
U & RealViformer   & 4.070 & 6.066 & 28.266 \\
\midrule
\multicolumn{5}{c}{\textbf{Diffusion-based Methods}} \\
\midrule
U & StableVSR*     & \textcolor{blue}{3.982} & \textcolor{blue}{6.122} & \textcolor{blue}{23.814} \\
\midrule
U & Ours           & \textcolor{red}{3.929} & \textcolor{red}{6.140} & \textcolor{red}{23.176} \\
\bottomrule
\end{tabular}}
\end{minipage}

\end{table*}

% \begin{table}[t]
% \vspace{-2mm}
% \caption{\textbf{Quantitative comparison on the VideoLQ dataset(bidirectional/offline).} 
% % We evaluate the no-reference quality of various VSR methods on the VideoLQ benchmark. Best and second-best results are highlighted in \textcolor{red}{red} and \textcolor{blue}{blue}, respectively.
% }
% \label{tab:vsr_online_comparison_videolq_bidirectional}
% \vspace{-4mm}
% \centering
% \small
% % \setlength{\tabcolsep}{2pt}
% \renewcommand{\arraystretch}{0.8}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{llccc}
% \toprule
% Dir. & Method & NIQE$\downarrow$ & NRQM$\uparrow$ & BRISQUE$\downarrow$ \\
% \midrule
% \multicolumn{5}{c}{\textbf{CNN-based Methods}} \\
% \midrule
% - & Bicubic        & 7.945 & 3.151 & 57.944 \\
% B & BasicVSR++     & 5.909 & 3.745 & 56.800 \\
% B & RealBasicVSR   & \textcolor{blue}{3.973} & 6.095 & 30.158 \\
% \midrule
% \multicolumn{5}{c}{\textbf{Transformer-based Methods}} \\
% \midrule
% B & RVRT           & 6.939 & 3.493 & 60.557 \\
% B & MIA-VSR        & 5.860 & 3.810 & 58.513 \\
% \midrule
% \multicolumn{5}{c}{\textbf{Diffusion-based Methods}} \\
% \midrule
% B & StableVSR      & \textcolor{blue}{3.973} &  \textcolor{red}{6.154} &  \textcolor{red}{22.973} \\
% B & MGLD-VSR       & 4.163 & 5.761 & 29.497 \\
% \midrule
% U & Ours           & \textcolor{red}{3.929} &  \textcolor{blue}{6.140} &  \textcolor{blue}{23.176} \\
% \bottomrule
% \end{tabular}%
% }
% \vspace{-2mm}
% \end{table}


==> tables/main/table_videoLQ_dit.tex <==
\begin{table}[h]
\centering
\small 
\caption{\textbf{Quantitative comparison with memory-intensive baselines on the VideoLQ dataset under a single RTX Pro 6000.}
\textcolor{gray}{Gray-shaded entries are reported from FlashVSR.} \texttt{--} indicates unavailable results.} 
\label{tab:videolq_dit}
\vspace{-3mm}
\setlength{\tabcolsep}{2pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccccccc}
\toprule
Dir. & Method & NIQE$\downarrow$ & NRQM$\uparrow$ & BRISQUE$\downarrow$ & Runtime (s) & \colorbox{yellow}{TTFF} (s) & Peak Mem (GB)\\
\midrule
B & VEhancer       & 6.221 & 3.85 & 48.1 & 9.544 & 477.237 & 47.985 \\
B & SeedVR2          & \textcolor{blue}{4.661} & \textcolor{blue}{5.523} & 37.975 & 1.126 & 56.28 & 76.094 \\
\rowcolor{black!10}
B & SeedVR2          & 5.205 & -- & -- & -- & -- & -- \\
B & UAV & 6.299 & 3.652 & 44.139 & 8.081 & 404.07 & 55.897 \\
\rowcolor{black!10}
B & UAV & 4.889 & -- & -- & -- & -- & -- \\
B & DOVE           & 5.090 & 5.214 & \textcolor{blue}{36.631} & 1.735 & 86.774 & 46.344 \\
U & FlashVSR & -- & -- & -- & -- & -- & OOM \\
\rowcolor{black!10}
U & FlashVSR & 3.803 & -- & -- & -- & -- & -- \\
U & FlashVSR-tiny & 4.569 & 5.164 & 42.514 & \textcolor{red}{0.204} & 1.224 & \textcolor{blue}{44.180} \\
\rowcolor{black!10}
U & FlashVSR-tiny & 4.070 & -- & -- & -- & -- & -- \\
U & Ours            & \textcolor{red}{3.929} & \textcolor{red}{6.140} & \textcolor{red}{27.176} & \textcolor{blue}{0.454} & \textcolor{red}{0.454} & \textcolor{red}{22.800} \\
\bottomrule
\end{tabular}%
}
\vspace{-4mm}
\end{table}

==> tables/main/table_videoLQ_unidirectional.tex <==
\begin{table}[t]
\vspace{-2mm}
\caption{\textbf{Quantitative comparison on the VideoLQ dataset(unidirectional/online).} 
% We evaluate the no-reference quality of various VSR methods on the VideoLQ benchmark. Best and second-best results are highlighted in \textcolor{red}{red} and \textcolor{blue}{blue}, respectively.
}
\label{tab:vsr_online_comparison_videolq_unidirectional}
\vspace{-4mm}
\centering
\small
% \setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{0.8}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llccc}
\toprule
Dir. & Method & NIQE$\downarrow$ & NRQM$\uparrow$ & BRISQUE$\downarrow$ \\
\midrule
\multicolumn{5}{c}{\textbf{CNN-based Methods}} \\
\midrule
- & Bicubic        & 7.945 & 3.151 & 57.944 \\
U & TMP            & 6.751 & 3.511 & 59.841 \\
\midrule
\multicolumn{5}{c}{\textbf{Transformer-based Methods}} \\
\midrule
U & RealViformer   & 4.070 & 6.066 & 28.266 \\
\midrule
\multicolumn{5}{c}{\textbf{Diffusion-based Methods}} \\
\midrule
U & StableVSR*     & 3.982 & 6.122 & 23.814 \\
\midrule
U & Ours           & \textcolor{red}{3.929} &  \textcolor{blue}{6.140} &  \textcolor{blue}{23.176} \\
\bottomrule
\end{tabular}%
}
\vspace{-2mm}
\end{table}

==> tables/main/table_vimeo90K_bidirectional.tex <==
\begin{table*}[t]
\caption{
\textbf{Quantitative comparison against bidirectional/offline methods on the Vimeo-90K-T dataset.} Stream-DiffVSR surpasses other bidirectional methods in perceptual quality, temporal consistency, and runtime. Runtime is the average per-frame inference time (seconds) on 448×256 videos using an RTX 4090. Best and second-best results are shown in \textcolor{red}{red} and \textcolor{blue}{blue}.}
\label{tab:vsr_online_comparison_vimeo_bidirectional}
\vspace{-3mm}
\centering
\small
\setlength{\tabcolsep}{3pt}
% \renewcommand{\arraystretch}{1.1}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llccccccccccccc}
\toprule
Dir. & Method & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & DISTS$\downarrow$ & MUSIQ$\uparrow$ & NIQE$\downarrow$ & NRQM$\uparrow$ & BRISQUE$\downarrow$ & VMAF$\uparrow$ & tLP$\downarrow$ & tOF$\downarrow$ & Runtime (s)$\downarrow$ & \colorbox{yellow}{TTFF} (s)$\downarrow$ \\
\midrule
\multicolumn{14}{c}{\textbf{CNN-based Methods}} \\
\midrule
-  & Bicubic & 29.282 & 0.864 & 0.297 & 0.209 & 23.433 & 8.735 & 3.588 & 61.714 & 42.928 & 11.606 & 2.49 & - & - \\
B  & BasicVSR++ & 37.479 & \textcolor{blue}{0.956} & 0.098 & 0.117 & 51.940 & 7.077 & 5.509 & 47.792 & 92.905 & \textcolor{blue}{4.691} & 1.57 & \textcolor{blue}{0.012} & 0.084 \\
B  & RealBasicVSR & 29.388 & 0.857 & 0.156 & 0.149 & \textcolor{blue}{56.986} & 5.069 & \textcolor{blue}{7.413} & 23.822 & 79.781 & 10.947 & 3.46 & \textcolor{red}{0.008} & \textcolor{blue}{0.056} \\
\midrule
\multicolumn{14}{c}{\textbf{Transformer-based Methods}} \\
\midrule
B  & RVRT & \textcolor{red}{37.815} & 0.955 & 0.093 & \textcolor{blue}{0.105} & 49.937 & 7.205 & 5.393 & 48.352 & \textcolor{blue}{94.660} & 4.873 & \textcolor{blue}{1.429} & 0.061 & 0.305 \\
B  & MIA-VSR & \textcolor{blue}{37.598} & \textcolor{red}{0.957} & \textcolor{blue}{0.086} & \textcolor{red}{0.101} & 51.402 & 7.116 & 5.569 & 47.865 & \textcolor{red}{95.113} & 4.696 & \textcolor{red}{1.419} & 0.096 & 0.672 \\
\midrule
\multicolumn{14}{c}{\textbf{Diffusion-based Methods}} \\
\midrule
B  & StableVSR & 31.823 & 0.878 & 0.095 & 0.111 & 54.582& \textcolor{blue}{4.745} & 7.265 & \textcolor{red}{20.039} & 86.936 & 26.224 & 3.108 & 5.749 & 40.243 \\
B  & MGLD-VSR & 29.651 & 0.865 & 0.151& 0.137 & \textcolor{red}{57.788} & 5.340 & 7.217 & \textcolor{blue}{20.761} & 71.509 & 12.550 & 4.661 & 5.426 & 27.130 \\
U  & Ours & 32.593 & 0.900 & \textcolor{red}{0.056} & \textcolor{blue}{0.105} & 52.755 & \textcolor{red}{4.403} & \textcolor{red}{7.672} & 29.297 & 88.311 & \textcolor{red}{4.307} & 2.689 & 0.041 & \textcolor{red}{0.041} \\
\bottomrule
\end{tabular}%
}
\end{table*}

==> tables/main/table_vimeo90K_dit.tex <==
\begin{table*}[t]
\caption{\textbf{Quantitative comparison with memory-intensive baselines on Vimeo-90K-T under a single RTX Pro 6000.}}
\label{tab:vsr_online_comparison_vimeo_dit}
\vspace{-3mm}
\centering
\small
\setlength{\tabcolsep}{3pt}
% \renewcommand{\arraystretch}{1.1}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llccccccccccccccc}
\toprule
Dir. & Method & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & DISTS$\downarrow$ & MUSIQ$\uparrow$ & NIQE$\downarrow$ & NRQM$\uparrow$ & BRISQUE$\downarrow$ & VMAF$\uparrow$ & tLP$\downarrow$ & tOF$\downarrow$ & Runtime (s)$\downarrow$ & \colorbox{yellow}{TTFF} (s)$\downarrow$ & Peak Mem (GB)\\
\midrule
B  & UAV & 25.263 & 0.72 & 0.226 & 0.177 & 55.562 & 5.602 & 7.247 & 24.766 & 46.489 & 9.546 & 7.576 & 0.499 & 3.490 & 37.987 \\
B  & SeedVR2 & 24.585 & 0.719 & 0.177 & 0.152 & \textcolor{blue}{58.809} & \textcolor{red}{4.204} & \textcolor{red}{8.107} & \textcolor{red}{20.447} & 41.430 & 21.191 & 12.460 & 0.039 & 0.270 & 41.366\\
B  & DOVE & \textcolor{blue}{28.611} & \textcolor{blue}{0.834} & \textcolor{blue}{0.12} & \textcolor{blue}{0.116} & 57.749 & 5.734 & 7.182 & \textcolor{blue}{23.388} & 77.997 & \textcolor{blue}{8.214} & \textcolor{blue}{4.387} & 0.223 & 1.560 & 31.934 \\
B  & VEnhancer & 23.712 & 0.712 & 0.234 & 0.189 & 57.822 & 6.175 & \textcolor{blue}{7.910} & 34.906 & 60.920 & 32.913 & 16.643 & 1.834 & 12.840 & 35.855 \\
U  & FlashVSR & 26.114 & 0.789 & 0.136 & 0.118 & \textcolor{red}{59.451} & 5.249 & 7.317 & 29.288 & \textcolor{blue}{78.575} & 19.018 & 9.351 & 0.025 & 0.150 & \textcolor{blue}{5.340}\\
U  & FlashVSR-tiny & 26.154 & 0.791 & 0.136 & 0.121 & 57.845 & 5.249 & 7.317 & 29.288 & 76.376 & 19.881 & \textcolor{blue}{9.793} & \textcolor{red}{0.019} & \textcolor{blue}{0.114} & \textcolor{red}{4.280}\\
U  & Ours & \textcolor{red}{32.593} & \textcolor{red}{0.900} & \textcolor{red}{0.056} & \textcolor{red}{0.105} & 52.755 & \textcolor{blue}{4.403} & 7.672 & 29.267 & \textcolor{red}{88.311} & \textcolor{red}{4.307} & \textcolor{blue}{2.689} & \textcolor{blue}{0.036} & \textcolor{red}{0.036} & 9.720\\
\bottomrule
\end{tabular}%
}
% \vspace{-2mm}
\end{table*}

==> tables/main/table_vimeo90K_unidirectional.tex <==
\begin{table*}[t]
\caption{
\textbf{Quantitative comparison against unidirectional/online methods on the Vimeo-90K-T dataset.}}
\label{tab:vsr_online_comparison_vimeo_unidirectional}
\vspace{-3mm}
\centering
\setlength{\tabcolsep}{3pt}
% \renewcommand{\arraystretch}{1.1}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llccccccccccccc}
\toprule
Dir. & Method & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & DISTS$\downarrow$ & MUSIQ$\uparrow$ & NIQE$\downarrow$ & NRQM$\uparrow$ & BRISQUE$\downarrow$ & VMAF$\uparrow$ & tLP$\downarrow$ & tOF$\downarrow$ & Runtime (s)$\downarrow$ & \colorbox{yellow}{TTFF} (s)$\downarrow$ \\
\midrule
\multicolumn{14}{c}{\textbf{CNN-based Methods}} \\
\midrule
-  & Bicubic & 29.282 & 0.864 & 0.297 & 0.209 & 23.433 & 8.735 & 3.588 & 61.714 & 42.928 & 11.606 & 2.49 & - & - \\
U  & TMP & \textcolor{red}{36.482} & \textcolor{red}{0.946} & 0.109 & 0.118 & 48.374 & 7.368 & 5.096 & 49.192 & 92.001 & \textcolor{blue}{4.870} & \textcolor{red}{1.603} & \textcolor{red}{0.006} & \textcolor{red}{0.006} \\
\midrule
\multicolumn{14}{c}{\textbf{Transformer-based Methods}} \\
\midrule
U  & RealViformer & 30.291 & 0.877 & 0.130 & 0.140 & 53.107 & 5.515 & 6.711 & \textcolor{blue}{24.628} & 54.689 & 8.232 & 2.769 & \textcolor{blue}{0.013} & 0.091 \\
\midrule
\multicolumn{14}{c}{\textbf{Diffusion-based Methods}} \\
\midrule
U  & StableVSR* & 31.729 & 0.875 & \textcolor{blue}{0.072} & \textcolor{blue}{0.113} & \textcolor{red}{54.447} & \textcolor{blue}{4.698} & \textcolor{red}{7.280} & \textcolor{red}{19.836} & 86.162 & 30.858 & 3.144 & 5.749 & 40.243 \\
U  & Ours & \textcolor{blue}{32.593} & \textcolor{blue}{0.900} & \textcolor{red}{0.056} & \textcolor{red}{0.105} & \textcolor{blue}{52.755} & \textcolor{red}{4.403} & \textcolor{blue}{7.672} & 29.297 & 88.311 & \textcolor{red}{4.307} & \textcolor{blue}{2.689} & 0.041 & \textcolor{blue}{0.041} \\
\bottomrule
\end{tabular}%
}
\end{table*}

==> tables/rebuttal/videoLQ.tex <==
% \begin{table}[t]
% \centering
% \small 
% \caption{\textbf{Quantitative comparison on the VideoLQ dataset under a single RTX A6000.} 
% % Since VideoLQ is a real-world dataset without paired ground truth, we report \emph{no-reference perceptual proxies} (MUSIQ, CLIP-IQA~\cite{wang2023exploring}) together with system-level efficiency metrics, including peak GPU memory, per-frame runtime, and maximum streaming latency. “OOM” denotes that the official implementation exceeds GPU memory limits under our evaluation setting; “--” indicates results unavailable due to OOM. Community UI variants with different engineering trade-offs (e.g., tiling or reduced precision) are not included for strict comparability.
% }
% \vspace{-3mm}
% \label{tab:rebuttal_videolq}

% \setlength{\tabcolsep}{2pt}  % 欄距壓到最小但可讀
% % \renewcommand{\arraystretch}{0.85} % 行距縮小但不重疊
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{lccccc}
% \toprule
% {Method} & {MUSIQ$\uparrow$} & {CLIP-IQA$\uparrow$} & {Peak Mem.} & {Per Frame Runtime (s)} & {Latency-max (s)} \\
% \midrule
% STAR\cite{xie2025starspatialtemporalaugmentationtexttovideo}            & -- & -- & OOM & -- & -- \\
% SeedVR\cite{wang2025seedvr}          & -- & -- & OOM & -- & -- \\
% SeedVR2\cite{wang2025seedvr2}          & -- & -- & OOM & -- & -- \\
% Upscale-A-Video\cite{zhou2024upscale} & -- & -- & OOM & -- & -- \\
% MGLD-VSR\cite{yang2024motion}         & 51.638 & 0.337 & 23.5 GB & 29.03 s & 289.94 s \\
% DOVE\cite{zhang2025dove}            & 48.334 & 0.364 & 42.344 GB & 1.16 s & 115.42 s \\
% Ours            & 45.242 & 0.316 & \textbf{21.8 GB} & \textbf{0.79 s} & \textbf{0.79 s} \\
% \bottomrule
% \end{tabular}%
% }
% % \vspace{-4mm}
% \end{table}

